An adaptive stochastic Galerkin tensor train discretization for randomly perturbed domains

A linear PDE problem for randomly perturbed domains is considered in an adaptive Galerkin framework. The perturbation of the domain's boundary is described by a vector valued random field depending on a countable number of random variables in an affine way. The corresponding Karhunen-Lo\`eve expansion is approximated by the pivoted Cholesky decomposition based on a prescribed covariance function. The examined high-dimensional Galerkin system follows from the domain mapping approach, transferring the randomness from the domain to the diffusion coefficient and the forcing. In order to make this computationally feasible, the representation makes use of the modern tensor train format for the implicit compression of the problem. Moreover, an a posteriori error estimator is presented, which allows for the problem-dependent iterative refinement of all discretization parameters and the assessment of the achieved error reduction. The proposed approach is demonstrated in numerical benchmark problems.

==> pgfplotsoptions.tex <==
%% create a new cycle list for egsz plots
\pgfplotscreateplotcyclelist{egsz color}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=square*},
  {brown!60!black,every mark/.append style={fill=brown!90!black},mark=otimes*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=diamond*},
}

\pgfplotscreateplotcyclelist{egsz color twocol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black!30}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black!30},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!70!black!30},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz bw twocol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!15}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!15},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!15},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz color threecol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=diamond*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=triangle*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=square*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=square*},
  }

\pgfplotscreateplotcyclelist{egsz bw threecol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!35}, mark=*},
  {black, every mark/.append style={fill=black!5}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!35},  mark=diamond*},
  {black,  every mark/.append style={fill=black!5},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!35},mark=triangle*},
  {black,every mark/.append style={fill=black!5},mark=triangle*},
  {black,every mark/.append style={fill=black},   mark=square*},
  {black,every mark/.append style={fill=black!35},mark=square*},
  {black,every mark/.append style={fill=black!5},mark=square*},
}  
  
\pgfplotscreateplotcyclelist{egsz color comparison}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black!50}, mark=square*},
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=triangle*},
}

\pgfplotscreateplotcyclelist{egsz color mi}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=diamond*},
}

\pgfplotscreateplotcyclelist{egsz bw mi}{%
  {black, every mark/.append style={fill=black}, mark=*},
  {black,  every mark/.append style={fill=black!35},  mark=square*},
  {black,every mark/.append style={fill=black!5},mark=diamond*},
}

%% set styles for general plots and error plots
\pgfplotsset{
  /tikz/tikzpic options/.style={
    scale=0.8,
  },
  egsz plot/.style={
    thin, % very thin, thin, semithick, thick, very thick
    %rounded corners=3pt,
    label style={font=\footnotesize}, %\tiny, \scriptsize, \footnotesize
    width=0.65\textwidth,
    height=0.3\textheight,
    grid=major, % none, major, minor, both
    legend columns=1,
    legend pos=south west,
    legend style={font=\tiny, rounded corners=2pt, cells={anchor=west}},
  },
  dof plot/.style={
    egsz plot,
    xlabel=mesh d.o.f.,
    xlabel style={yshift=0.5em},
  },
  %
  right side/.style={
    ylabel=,
  },
  %
  top label/.style={
    legend pos=north west,
  },
  %
  wide label/.style={
    legend columns=3,
  },
  sol error plot/.style={
  dof plot,
  cycle list name=egsz bw twocol,
  ylabel=relative mean error: $\norm{e}$,
  },
  %
  sol error plot dbl 1/.style={
  dof plot,
  width = 0.48\textwidth,
  cycle list name=egsz bw twocol,
  ylabel=relative mean error: $\norm{e}$,
  },
  sol error plot dbl 2/.style={
  dof plot,
  width = 0.48\textwidth,
  cycle list name=egsz bw twocol,
  ylabel=,
  },
  %
  estimator efficiency plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error: $\norm{e}$,
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  estimator efficiency plotb/.style={
    dof plot,
    cycle list name=egsz bw threecol,
    legend columns=3,
    ylabel=efficiency index,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend to name=efflegend,
    mark options={scale=0.75},
    legend style={mark options={scale=0.75}},
  },
  estimator efficiency plotc/.style={
    estimator efficiency plot,
    legend pos=north west,
  },
  %
  error multiindex plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error (multi-indices),
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  %
  cells multiindex plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=cells/multi-indices,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend pos=north west,
  },
  %
  error comparison plot/.style={
    dof plot,
    cycle list name=egsz bw twocol,
    ylabel=energy error: $\norm{e}$,
    ylabel style={yshift=-1.9ex,xshift=1em},
  },
  %
  mi error plot/.style={
    dof plot,
    cycle list name=egsz bw mi,
    ylabel=number multi-indices,
    ylabel style={yshift=-1.9ex,xshift=1em},
    xlabel=energy error,
    legend pos=north east,
    legend columns=1,
  },
  estimator comparison plot/.style={
    dof plot,
    width=0.45\textwidth,
    legend columns=3,
    cycle list name=egsz bw threecol,
    ylabel=,
    ylabel style={yshift=-1.9ex,xshift=1em},
    legend to name=legend,
    mark options={scale=0.75},
    legend style={mark options={scale=0.75}},
  },
}

\tikzset{slopetriangle/.style={
    bottom color=black!20,
    middle color=black!5,
    top color=white,
    draw=black}
    }

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 

